Chain-Free String Constraints (Technical Report)

We address the satisfiability problem for string constraints that combine relational constraints represented by transducers, word equations, and string length constraints. This problem is undecidable in general. Therefore, we propose a new decidable fragment of string constraints, called weakly chaining string constraints, for which we show that the satisfiability problem is decidable. This fragment pushes the borders of decidability of string constraints by generalising the existing straight-line as well as the acyclic fragment of the string logic. We have developed a prototype implementation of our new decision procedure, and integrated it into in an existing framework that uses CEGAR with under-approximation of string constraints based on flattening. Our experimental results show the competitiveness and accuracy of the new framework.

==> sections/app.thm-chainfree.tex <==
%\section{Proof of Theorem \ref{thm-chainfree}}
%\label{app.thm-chainfree}

%\smallskip

\noindent
{\em Base Case ({\bf B=0}).} Thus there is no benign chain in $G_{\formula}$ and so  Theorem \ref{thm-chainfree}  holds.

\smallskip

\noindent
{\em Induction Case ({$\bf B>0$}).}
Let us start by showing how to remove one benign chain (and the set of relational constraints labelling it) in the case where the splitting graph of $\formula$ does not contain nested chains. Let $\rho = (\pos_0,\pos_1),(\pos_1,\pos_2),\ldots,(\pos_n,\pos_0)$ be a benign chain in the splitting graph $G_\formula$. For every $i \in \{0,\ldots,n\}$, let $\relconstrof {x_i} {t_{i}} {\rel_i}$ be the length preserving relation constraint to which the position $\pos_i$ belongs. We assume w.l.o.g.\footnote{This is possible since   if there is benign chain that uses only right positions then there exists also a  benign chain that uses only left positions.} that all the positions $\pos_0, \pos_1,\ldots, \pos_n$ are left positions. Since $\rho$ is a benign chain, the variable $x_i$ is appearing in the string term $t_{(i-1) \mod (n+1)}$ for all  $i \in \{0,\ldots,n\}$. Furthermore, we can use the fact that the relational constraints are length preserving to deduce that the string-values of variables $x_0,x_1, \ldots, x_n$ must have the same length (it is a crucial insight for the proof). This  implies also that, for every $i \in \{0,1,\ldots,n\}$, the string term $t'_i$, that is constructed by removing from $t_i$ one occurence of the variable $x_{(i+1) \mod (n+1)}$, is equivalent to the empty word. Therefore,  the relational constraint  $\relconstrof {x_i} {t_{i}} {\rel_i}$ can be rewritten as 
 $\relconstrof {x_i} {x_{(i+1) \mod (n+1)}} {\rel_i}$ for all $i \in \{0,1,\ldots,n\}$.
 
Let $x_{i_1},x_{i_2},\ldots, x_{i_k}$ be the maximal subsequence of pairwise distinct variables in
$x_0,x_1,\ldots,x_n$. Let ${\tt index}$ be a  mapping that associates to each index $\ell \in
\{0,\ldots,n\}$, the index $j \in \{1,\ldots,k\}$  such that $x_\ell=x_{i_j}$. We can  transform the
transducer $\rel_i$, with $i \in \{0,\ldots,n\}$, to a length preserving $k$-tape automaton $A_i$
such that a word $(w_1,w_2,\ldots,w_k) $ is accepted by $A_i$ if and only if $(w_{{\tt
index}(i)},w_{{\tt index}((i+1) \mod (n+1))})$ is accepted by $\rel_i$. Then, let $A$ be the $k$-tape
automaton resulting from the intersection of $A_0,\ldots, A_n$. Observe that $A$ is also a
length-preserving automaton. Furthermore, we have that $(w_1,w_2,\ldots,w_k) $ is accepted by $A$ if
and only if $(w_{{\tt index}(i)},w_{{\tt index}((i+1) \mod (n+1))})$ is accepted by $\rel_i$ for all
$i \in \{0,\ldots,n\}$ (i.e., the automaton $A$ characterizes all possible solutions of
$\bigwedge_{i=0}^n \relconstrof {x_i} {x_{(i+1) \mod (n+1)}} {\rel_i}$). Ideally, we would like to
replace the $\bigwedge_{i=0}^n \relconstrof {x_i} {x_{(i+n) \mod (n+1)}} {\rel_i}$ by
$A(x_{i_1},x_{i_2},\ldots, x_{i_k})$ however our syntax forbids such $k$-ary relation.  To overcome
this problem, we first extend our alphabet $\Sigma$ by all the letters in $\Sigma^k$ and then we
replace  $\bigwedge_{i=0 }^n\relconstrof {x_i} {x_{(i+1) \mod (n+1)}} {\rel_i}$ by  $\varphi:= A(x)
\wedge \bigwedge_{j=1 }^k\relconstrof {x_{i_j}} {x} {\pi_j}$ where $x$ is a fresh variable and  for
every $j \in \{1,\ldots,k\}$, $\pi_j$ is the length preserving transducer  that accepts all pairs of
the form $(w_j,(w_1,w_2,\ldots,w_k))$. Finally, let $\formula'$ be the formula obtained from
$\formula$ by replacing the subformula $\bigwedge_{i=0}^n \relconstrof {x_i} {t_{i}} {\rel_i}$ in
$\formula$ by $\varphi \wedge |t'_i|=0$ (remember that the string term $t'_i$ is  $t_i$ with one
occurence of the variable  $x_{(i+1) \mod (n+1)}$ removed).  It can be seen from the discussion above
that $\bigwedge_{i=0}^n \relconstrof {x_i} {t_{i}} {\rel_i}$ is equivalent to $\exists x:\varphi
\wedge |t'_i|=0$ (both say that $\relconstrof {x_i} {x_{(i+1) \mod (n+1)}} {\rel_{i}}$ holds for all
$i\in\{0,\ldots, n\}$ and that values of all the other variables occurring in $t_0,\ldots,t_n$ must be
$\epsilon$). Hence $\formula'$ and $\formula$ are equisatisfiable. Furthermore, the number of
relational constraints that are labelling the set of benign chains in the \mbox{splitting graph} of
$\formula'$ is strictly less than  ${\bf B}$ (since $\pi_j$ cannot label any benign chain in
$\formula'$).




Let us now consider the case where the splitting graph of $\formula$ contains nested benign chains.
Let $\rho = (\pos_0,\pos_1),(\pos_1,\pos_2),\ldots,(\pos_n,\pos_0)$ be a benign chain in the
splitting graph $G_\formula$. We assume w.l.o.g. that all the positions $\pos_0, \pos_1,\ldots,
\pos_n$ are left positions. Let $S$ be \emph{the smallest} set of positions in $G_\formula$
satisfying that: (1) $\{\pos_0,\pos_1,\ldots,\pos_n\}$ is a subset of $S$, and (2) $S$ includes all
positions of every benign chain that traverses a position $\pos \in S$. Assume that $S =
\{q_0,q_1,\ldots,q_m\}$, and  observe that all the positions in $S$ are left positions and for each
pair of positions $q_i$ and $q_j$, there is a path in the graph  $G_\formula$ from $q_i$ to $q_j$.
For every $i \in \{0,\ldots,m\}$, let $\relconstrof {x_i} {t_{i}} {\rel_i}$ be the length preserving
relation constraint to which the position $q_i$ belongs. Using a similar reasoning as in the case of
non-nested chains, we can deduce that all the string-values of variables $x_i$ must have the same
length. Let $y_i$ be the {\em unique} string variable in $\{x_0,x_1,\ldots,x_m\}$ that appears in
$t_i$ and let the rest of $t_i$, i.e. $t_i$ with $y_i$ removed, be denoted $t_i'$ (The uniqueness of $y_i$ can be assumed without loss of generatity. Observe that if there were
multiple occurrences of variables from $\{x_0,x_1,\ldots,x_m\}$ in $t_i$, then, since their values
must have the same lenght as that of $x_i$, the only lenght possible was $0$, i.e. all variables
$x_0,x_1, \ldots,x_m$ must be assigned $\epsilon$. We could replace them in $\formula$ by $\epsilon$
and remove $\bigwedge_{i \in \{0,\ldots,m\}} \relconstrof {x_i} {t_{i}} {\rel_i}$ from $\formula$.).  
%Let  $t'_i$ be the string term constructed from $t_i$ by removing all variables but $y_i$. 
Notice that all variables of each $t_i$ other then $y_i$ must be valuated by $\epsilon$, because, again, the relatios are lenght preserving and the constraints are left-sided. 
%from $t_i$ the variable $y_i$, is equivalent to the empty word. 
Therefore, these variables can be removed from the terms and each relational constraint  $\relconstrof {x_i} {t_{i}} {\rel_i}$, $i \in \{0,1,\ldots,m\}$, can be rewritten as 
$\relconstrof {x_i} {y_i} {\rel_i}$. 
 
 
Next, we can proceed in similar manner as in the case of non-nested chains. Let $x_{i_1},x_{i_2},\ldots, x_{i_k}$ be the maximal subsequence of pairwise distinct variables among  $x_0,x_1,\ldots,x_m$. Let ${\tt index}_x$ (resp. ${\tt index}_y$) be a  mapping that associates to each index $\ell \in \{0,\ldots,m\}$, the index $j \in \{1,\ldots,k\}$  such that $x_\ell=x_{i_j}$ (resp. $y_\ell=x_{i_j}$). We can  transform the transducer $\rel_i$, with $i \in \{0,\ldots,m\}$, to a length preserving $k$-tape automaton $A_i$ such that a word $(w_1,w_2,\ldots,w_k) $ is accepted by $A_i$ if and only if $(w_{{\tt index}_x(i)},w_{{\tt index}_y(i)})$ is accepted by $\rel_i$. Let $A$ be the length preserving $k$-tape automaton resulting from the intersection of $A_0,\ldots, A_m$. Then, we have that $(w_1,w_2,\ldots,w_k) $ is accepted by $A$ if and only if $(w_{{\tt index}_x(i)},w_{{\tt index}_y(i)})$ is accepted by $\rel_i$ for all $i \in \{0,\ldots,m\}$ (i.e., the automaton $A$ characterizes all possible solutions of $\bigwedge_{i=0 }^m\relconstrof {x_i} {y_i} {\rel_i}$). 
Now, we are ready to transform the subformula $\bigwedge_{i=0} ^m\relconstrof {x_i} {y_{i}} {\rel_i}$ in $\formula$ into a chain-free formula. To do that,  we first  extend our alphabet $\Sigma$ by all the letters in $\Sigma^k$ and then we replace  $\bigwedge_{i= 0}^m\relconstrof {x_i} {y_i} {\rel_i}$ by  $\varphi:= A(x) \wedge \bigwedge_{j\in \{1,\ldots,k\} }\relconstrof {x_{i_j}} {x} {\pi_j}$ where $x$ is a fresh variable and  for every $j \in \{1,\ldots,k\}$, the transducer $\pi_j$ is  defined as in the non-nested case. Finally, let $\formula'$ be the formula obtained from $\formula$ by replacing the sub-formula $\bigwedge_{i \in \{0,\ldots,n\}} \relconstrof {x_i} {t_{i}} {\rel_i}$ in $\formula$ by $\varphi \wedge |t'_i|=0$ (remember that is the string term $t'_i$ is  $t_i$ from which we have removed one variable  from $\{x_0,x_1,\ldots,x_m\}$). Now we are ready to state our lemma:

\begin{lemma}
\label{removingchains}
The formula $\formula$ is satisfiable if and only if the formula   $\formula'$ is satisfiable. Furthermore, if $\sigma:=(s_0,s_1),(s_1,s_2),\ldots,(s_\ell,s_0)$ is a chain in  the splitting graph of $\formula'$ then $\sigma$ is also a chain in the splitting graph of $\formula$.\end{lemma}

\input{sections/proof_L2}


As a corollary of the above lemma, we obtain that the new relation $\pi_j$ cannot be part of any benign chain. Thus, the number of relational constraints that are labelling the set of benign chains in the \mbox{splitting graph} of $\formula'$ is strictly smaller than  ${\bf B}$ (since $\pi_j$ cannot be used to label any benign chain in $\formula'$).



==> sections/experiments_extra.tex <==
\section{Extra Experiments}
\label{section:extra_experiments}
\input{sections/fig.results_extra} 

In this section, we carry more experiment on other suites such as Kaluza, AppScan, and PISA. These suites have been executed successfully by \Trau and CVC4 in their previous work. Our aim of carrying extra experiment is to guarantee that our new decision procedure does not have negative effect on  \Trauplus. The Table \ref{fig:extra_results} shows that \Trauplusspace is also successful in solving these suites. 

\medskip

%\noindent
{\it Kaluza suite.} The Kaluza suite \cite{Saxena10:kaluza} is generated by a JavaScript symbolic execution engine. It consists of 47284 test cases, including length, regular and (dis)equality constraints. For this suite, Ostrich returns unknown for 8889 cases. We contacted Ostrich' authors and received the explanation that those cases fall out from straight line fragment. CVC4 times out on 35 cases. Z3-str3 times out on 350 cases and cannot answer on 640 cases. \Trau and \Trauplusspace have the same performance, which is better than the other solvers as they time out  only in 6 cases.  
\medskip

%\noindent
{\it PISA and AppScan suite.} The PISA suite includes constraints from real-world Java sanitizer methods that were used in the evaluation of the PISA system \cite{Tateishi:2013:PIS:2522920.2522926}. The suite has 12 tests, including transducer constraints such as Substring, IndexOf, and Replace operations. The AppScan suite is derived from security warnings output by IBM Security AppScan Source Edition \cite{AppScan}. The suite has 8 tests, including  transducer constraints and (dis)equality constraints. In both suites, the performance of CVC4, Z3-str3, \Trau, and \Trauplusspace are able to solve all test cases.   

%	{\it PISA and AppScan suite.} The PISA suite includes constraints from real-world Java sanitizer methods that were used in the evaluation of the PISA system \cite{Tateishi:2013:PIS:2522920.2522926}. The suite has 12 tests, including transducer constraints such as Substring, IndexOf, and Replace, and (dis)equality constraints. The AppScan suite is derived from security warnings output by IBM Security AppScan Source Edition \cite{AppScan}. The suite has 8 tests, including regular membership constraints, transducer constraints and (dis)equality constraints.
%	The experimental results are summarised in Table~\ref{fig:kaluzaresults}. In both suites, the performance of  \Trau is comparable to Z3-str3 (they  are able to solve all test cases). CVC4 times out on 1 test case in each suite.  {\sc Trau} cannot run these two suites since it does not support transducer constraints. 

==> sections/fig.results_extra.tex <==
\newcolumntype{g}{>{\columncolor{white!20}}l}
\begin{table*}[h]
\centering
%\rowcolors[]{2}{gray!20}{white}
\normalsize{
\begin{tabular}{|g|l|>{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}p{1.5cm}|}
\hline
\rowcolor{white}						&				& Ostrich			& Z3-str3	& CVC4		& {\sc Trau} 	& \Trauplus \\ \hline	

\rowcolor{gray!20}\cellcolor{white}		&	sat        	& 28523				& 34495		& 35235			& 35246     	& 35246 \\ 
\rowcolor{gray!20}\cellcolor{white}		&	unsat		& 9872      			& 11799		& 12014 		& 12014      	& 12014 \\ 
										&	timeout     & 0		            & 350		& 35  			& 6	     		& 6 \\  
\multirow{-4}{*}{{\bf Kaluza} (47284)}	& error/unknown & 8889              & 640		& 0  			& 0	   			& 0 \\ \hline  
\rowcolor{gray!20}\cellcolor{white}		&	sat        	& 2             	& 8			& 8				& 8     	 	& 8\\ 
\rowcolor{gray!20}\cellcolor{white}		&	unsat		& 0             	& 0			& 0     		& 0     	 	& 0\\ 
										&	timeout     & 0              	& 0			& 0         	& 0	    		& 0\\  
\multirow{-4}{*}{{\bf Appscan} (8)}		& error/unknown & 6              & 0			& 0           	& 0	     	 	& 0\\ \hline  
\rowcolor{gray!20}\cellcolor{white}		&	sat        	& 0		        	& 8			& 8				& 8      		& 8\\ 
\rowcolor{gray!20}\cellcolor{white}		&	unsat		& 0           	  	& 4			& 4     		& 4     	 	& 4\\ 
										&	timeout     & 0              	& 0			& 0          	& 0	    		& 0\\  
\multirow{-4}{*}{{\bf PISA} (12)}		& error/unknown & 12            		& 0			& 0           	& 0	     		& 0\\ \hline \hline  
\rowcolor{gray!20}\cellcolor{white}		&	solved      	& 39387            	& 46314		& 47269			& 47298     	& 47298\\ 
\multirow{-2}{*}{{\bf Total} (47304)}	& 	unsolved 	& 8907           & 990		& 35           	& 6	     	 	& 6\\ \hline   
\end{tabular}
}

\caption{
\normalsize{Results of running each solver over Kaluza, Appscan, and PISA suites.  }
}
%\vspace{-0.4cm}
\label{fig:extra_results} 
\end{table*}











==> sections/fig.syntax.tex <==
\begin{tikzpicture}[framed,background rectangle/.style={thick,draw=black,rounded corners,fill = green!5}, scale=1, transform shape]
%\small
\node (species1) {
		%\begin{tabular}{r c l r} 
		%$\constrs$ 		& ::= & 		$\constr$ $|$ $\constrs \wedge \constrs$\\
		%$\constr$ 		& ::= & 		$\constr_{s}$ $|$ $\constr_{i}$ $|$ $\constr_{t}$ $|$ $\constr_{g}$\\
		%$\constr_{s}$ 	& ::= & 		$\term_{s} = \term_{s}$ $|$ $\term_{s} \neq \term_{s}$ \\
		%$\constr_{t}$ 	& ::= & 		$\term_{s} \in \transducerof{\term_{s}}$ \\
		%$\constr_{g}$ 	& ::= & 		$\term_{s} \in \cfg$ \\
		%$\constr_{i}$ 	& ::= & 		$\term_{i} \geq \term_{i}$ 	\\
		%$\term_{s}$		& ::= &  	$w$ 	$|$ $x$ 	$|$ 	$\term_{s} \app \term_{s}$														& \\
		%$\term_{i}$		& ::= &		$\lengthof{\term_s}	$ $|$ $k$	 \\					
		%\end{tabular}
$
		\begin{array}{c @{\,::=\ } l } 
		\formula 		& 		\constr \mid \formula \wedge \formula \mid \formula \vee \formula \mid \neg\formula\\
		\constr 			& 		\memconstrof \strterm \automaton \mid \relconstrof \strterm \strterm   \rel \mid \arterm \geq \arterm  \\ 
		\rel 	   		&	   \transducer \mid {=} \\
		\strterm			&     \emptystr \mid	x \mid \strterm \concat \strterm\\														
		\arterm 			&		k \mid \lengthof{\strterm} \mid \arterm + \arterm 	 					
		\end{array}
$
};
\end{tikzpicture}


==> sections/figure2.tex <==
\begin{tikzpicture}[rotate=90,framed,
background rectangle/.style={thick,draw=black,rounded corners,fill = green!5}, 
scale=0.7, state/.style={fill=blue!20, draw, circle, semithick, minimum width=0.5cm, inner sep=0pt, text centered, font = \large \sffamily},transform shape]
  [auto,
  	->,>=stealth',shorten >=2pt,auto,node distance=2cm,on grid,semithick  	
	]

%\node[state] (x)							{\large \sffamily x};
%\node[state] (y)	[below right=1cm of x]	{\large \sffamily t2};
%\node[state] (z)	[above right=1cm of x]	{\large \sffamily z};

\matrix [row sep=0.55cm, column sep = 0.25cm]
%{	\node [state] (x) {x}; 	& \node [state] (y) {y};		 		\\ 
%	\node [state] (y1) {y}; & \node [state] (t1) {t};		 		\\ 
%	\node [state] (z1) {z}; & \node [state] (t2) {t};\\
%	 								& \node [state] (x1) {x};\\ 
%};
{	
	\node [state] (x) {x}; &\node [state] (z1) {z}; & \node [state] (y1) {y}; \\
	\node [state] (y) {y}; & \node [state] (x1) {x}; & \node [state] (u1) {u}; & \node [state] (v1) {v};\\
};

\path[-, thick, color=red,->] (x) edge			[bend right]		node{} 		 (y);	
\path[-, thick, color=red,->] (y) edge			[bend right]		node{}		 (x);	
\path[-, thick, color=red,->] (y1) edge		[bend right]		node{}		 (x1);	
\path[-, thick, color=red,->] (x1) edge		[bend right]		node{}		 (y1);	
\path[-, thick, color=blue,->] (z1) edge		[bend right]		node{}		 (x1);	
\path[-, thick, color=blue,->] (u1) edge		[bend right]		node{}		 (y1);	
\path[-, thick, color=blue,->] (v1) edge		[bend right]		node{}		 (y1);	
\end{tikzpicture}


==> sections/proof_L2.tex <==
%\section{Proof of Lemma~\ref{removingchains}}
\begin{proof}
The proof of the equisatisfiability between $\formula$ and $\formula'$ is an immediate consequence
of the construction. Let us prove by contradiction the second part of the lemma. Let us assume that
there is a chain $\sigma:=(s_0,s_1),(s_1,s_2),\ldots,(s_\ell,s_0)$ in the splitting graph of
$\formula'$ that is not a chain in the splitting graph of $\formula$. This means that at least one
of the edges of the chain $\sigma$ is labelled by a relational constraint in $\varphi$ (i.e.,
$\{\pi_1, \pi_2,\ldots,\pi_k\} \cap \{\edgecons(s_0,s_1),\edgecons(s_1,s_2),
\ldots,\edgecons(s_\ell,s_0) \}\neq \emptyset$). On the other hand, there must be edges labeled by constraints other than $\pi_o,1\leq o \leq k$ since $G_\varphi$ cannot have a chain, by definition.
%
%Let $j \in \{0,1,\ldots,\ell\}$  (resp. $j' \in
%\{0,1,\ldots,\ell\}$) be the smallest (resp. largest) index such that $\edgecons(s_j,s_{(j+1) \mod
%(\ell+1)})$ (resp. $\edgecons(s_{j'},s_{({j'}+1) \mod (\ell+1)})$) is in  $\{\pi_1,
%\pi_2,\ldots,\pi_k\}$. 
%
%Let $j \in \{0,1,\ldots,\ell\}$ be the smallest index such that $\edgecons(s_j,s_{(j+1) \mod
%(\ell+1)})\in\{\pi_1,
%\pi_2,\ldots,\pi_k\}$ and 
%let $j' \in
%\{0,1,\ldots,\ell\}$ be the largest such index. 
%
Let $j,j'\in \{0,\ldots,\ell+1\}$ mark the borders of a maximum sub-sequence of the chain $\{(s_{j},s_{(j+1) \mod (\ell+1)}),(s_{(j+1) \mod (\ell+1)},s_{(j+2) \mod (\ell+1)}), \ldots,(s_{(j'-1) \mod (\ell+1)},s_{j'})$ in which constraints on all edges are in $\{\pi_1, \pi_2,\ldots,\pi_k\}$.
%\footnote{Note that $j+\ell \mod (\ell +1)$ is equivalent to $(j-1) \mod (\ell+1)$.}.
%
%Let $j \in \{0,1,\ldots,\ell\}$ be an index such that 
%$\edgecons(s_j,s_{(j+1) \mod (\ell+1)})\in\{\pi_1, \pi_2,\ldots,\pi_k\}$ and 
%$\edgecons(s_{(j+\ell) \mod (\ell+1)},s_{j})\not\in\{\pi_1,\pi_2,\ldots,\pi_k\}$.\footnote{Note that $j+\ell \mod (\ell +1)$ is equivalent to $(j-1) \mod (\ell+1)$.}
%Let $j' \in
%\{0,1,\ldots,\ell\}$ be the index such that 
%$\edgecons(s_{j'+1 \mod (\ell+1)}\not\in\{\pi_1,\pi_2,\ldots,\pi_k\})$ and has 
%the minimum distance from $j$, where the distance from $j$ is the number $d\in\{0,\ldots,\ell\}$ such that $j' = (j+d) \mod (\ell +1)$ 
% (that is, $s_j$ and $s_{j'}$ are the borders of a maximum interval of the chain, modulo $\ell+1$, where all constraints are in $\{\pi_1, \pi_2,\ldots,\pi_k\}$). 
%
%Let us assume that $\pi_i:= \edgecons(s_j,s_{(j+1) \mod (\ell+1)})$ (resp.
%$\pi_{i'}:= \edgecons(s_{j'},s_{({j'}+1) \mod (\ell+1)})$).  
%
Assume that $\pi_i:= \edgecons(s_j,s_{(j+1) \mod (\ell+1)})$ and 
$\pi_{i'}:= \edgecons(s_{j'},s_{({j'}+1) \mod (\ell+1)})$.  
%
%It is easy to see that $\nodevar(s_j)=x_i$  (resp. $\nodevar(s_{j'})=x$). 
%
It is easy to see that $\nodevar(s_j)=x_i$ and $\nodevar(s_{j'})=x$ (since positions with $x$ appear only in constraints $\pi_o(x_o,x)$, i.e., edges from or to $x$ may only be labeled by some $\pi_o$, and these cannot lead to $s_j$ or from $s_{j'}$ by definition of $j$ and $j'$). 
%
This means that the  position $s_j$ is a left
position and corresponds to the variable $x_i$ while the position $s_{j'}$ is a right position and
corresponds to the fresh variable $x$. Observe that $\nodevar({s_{(j'+1) \mod (\ell+1)}})=x_{i'}$.
Furthermore, we know that the position $s_{(j-1) \mod (\ell+1)}$ belongs to the splitting graph
$G_{\formula}$ (as well as to $G_{\formula'}$). This implies that $s_{(j-1) \mod (\ell+1)}$ is not in the set $S$ (otherwise it will
not belong to the graph $G_{\formula'}$). By definition, the podgraf of $G_\formula$ induced by $S$ is strongly connected. Therefore, there is
a path $(q_{j_0},q_{j_1}),(q_{j_1},q_{j_2}),\ldots,(q_{j_{r-1}},q_{j_r})$ in $G_\formula$, that uses only positions in $S$, such that $\nodevar{(q_{j_0})}=x_i$ and
$\nodevar{(q_{j_r})}= x_{i'}$. Then, by
replacing the path $(s_{(j-1) \mod (\ell+1)},s_j)(s_j,s_{(j+1) \mod (\ell+1)}),\ldots ,(s_{j'
},s_{(j'+1) \mod (\ell+1)})$  in  $\sigma$  by $(s_{(j-1) \mod
(\ell+1)},q_{j_0}),(q_{j_0},q_{j_1}),(q_{j_1},q_{j_2}),\ldots,  (q_{j_{r-1}},s_{(j'+1) \mod
(\ell+1)})$, we obtain another chain $\sigma'$. Since $\sigma'$ is a chain in
$G_{\formula}$, it is a benign chain. Since $\sigma'$ traverses some
positions in $S$, all the positions of $\sigma'$ are in $S$
including the position $s_{(j-1) \mod (\ell+1)}$, which is a contradiction.\qed
\end{proof}




==> sections/termination-proof-lukas.tex <==



\section{Proof of Theorem~\ref{theorem:splitting}}
\label{section:termination}
We will start by showing the most crucial property of splitting which is that it preserves chain-freeness.
\begin{lemma} 
\label{lemma:chain-free}
Splitting steps preserve chain-freeness.
\end{lemma}
\begin{proof}
Let us assume that a clause $\clause'$ be obtained from a chain-free clause $\clause$ by a left split. We omit the case of a right split as it is analogous.
Creation of $\clause'$ from $\clause$ might be understood as a sequence of two steps.
The first is construction of $\clause[x/x_1\concat x _2]$,
the second is replacement of the constraint $\relconstrof {x\concat\term} {y\concat\term'}[x/x_1 \concat x_2] \rel$
by the conjunction $\relconstrof {x_1} {y} {R_i}\land \relconstrof {x_2\concat\term} {\term'} {\rel_i'}$ 
(for some $i$, see the definition of left split).
When reasoning modulo isomorphism of graphs, then the second step only removes edges (the positions of the new left conjunct now cannot use the positions of the new right conjunct as the intermediate positions for creating edges and vice versa).
Therefore the chain must have been created during the first step, the substitution, and must be present already in  $\clause[x/x_1\concat x _2]$. 
Notice that the splitting graph of $\clause[x/x_1\concat x _2]$ with positions labeled by  $x_1$ removed is isomorphic to the original graph $G_\clause$, as well as when $x_2$ is removed. Therefore, since  $G_\clause$ does not contain a chain, the new chain must contain positions labeled by $x_1$ as well as positions labeled by $x_2$.
%Consider such path in $p_1,\ldots,p_n$ in $G_{\clause[x/x_1\concat x _2]}$ where $p_1$ is labeled by $x_1$ and $p_n$ by $x_2$. 
Since $x_1$ and $x_2$ are fresh variables that were introduced by substitution of $x$, 
they always appear in a side of a constraint together. 
Therefore, by the definition of the edges of a splitting graph $G_{\clause[x/x_1\concat x _2]}$,  
for every pair of edges $(p_1,p_2)(p_2,p_3)$ with the label of $p_2$ being $x_1$, 
there is a pair of edges $(p_1,p_2')(p_2',p_3)$ with $x_2$ being the label of $p_2'$. 
We can therefore replace all occurrences of $x_1$ in the chain by occurrences of $x_2$, and obtain a chain in $G_{\clause[x/x_1\concat x _2]}$ where only $x_2$ occurs. 
This is however a contradiction with the fact derived above that any new cycle must have contain both $x_1$ and $x_2$.
\qed
\end{proof}

\paragraph{Successor relation.}
We will first introduce some notation related to splitting steps.
Recall that split of a relational constraint $\constr \defeq \relconstrof {x\concat\term} {y\concat\term'} \rel$ 
is the formula 
$\leftsplit \lor \rightsplit$ where
\begin{eqnarray*}
\leftsplit  \defeq & \bigvee\nolimits_{i=1}^n \relconstrof {x_1} {y} {R_i}\land \relconstrof {x_2\concat\term} {\term'} {R_i'} \ [x/x_1\concat x_2]\\
\rightsplit  \defeq & \bigvee\nolimits_{j=1}^m \relconstrof x {y_1}{R_j}\land \relconstrof {\term}{y_2\concat\term'} {R_j'} \ [y/y_1\concat y_2]
\end{eqnarray*}
$n,m\in\nat$,  $x_1,x_2,y_1,y_2$ are fresh variables (and one of the disjunct can be omited if $t$ or $t'$ equals $\emptystr$).
The right sides of the resulting constraints are the successors of the right side of the original constraint, and likewise the left sides of the resulting constraints are successors of the left side of the original constraint. 
%
Further, consider a splitting step that is applied to a clause $\clause \defeq \constr\land \formula$ where $\constr\defeq \rel(x\concat\term,y\concat\term')$
and that creates a DNF of the disjunction
$$
(\leftsplit\land\formula[x/x_1\concat x_2]\land |x| = |x_1| + |x_2|) \lor (\rightsplit \land\formula[y/y_1\concat y_2] \land |y| = |y_1| + |y_2|)
$$ 
where $\leftsplit$ and $\rightsplit$ are the left and the right split, respectively, of $\constr$.
Besides the successor relation on sides of constraints defined above, 
for every original constrain $\constr'$ of $\formula$,
the left sides of the constraints $\constr'[x/x_1\concat x_2]$ and $\constr'[y/y_1\concat y_2]$ are the successors of the left side of $\constr'$, and likewise   
the right sides of the constraints $\constr'[x/x_1\concat x_2]$ and $\constr'[y/y_1\concat y_2]$ are the successors of the right side of $\constr'$.
\medskip




%
We will continue by showing that Phase 1 terminates. 
Let $\clause$ be a clause that appears during Phase~1. 
%
For a root constraint $\rel(t,t')$ of $H_\clause$, 
its \emph{outer side} is the one from $t$ and $t'$ which consists exclusively of root positions of $H_\clause$,
and the side which is not outer (if there is one) is called the \emph{inner side}.
The termination proof will use several auxiliary observations:
\begin{lemma}
\label{lemma:aux1}
For every clause $\clause$ that appears during Phase 1 and for every clause $\clause'$ created from it by splitting, it holds that:
\begin{enumerate}
\item \label{lemma:root}
Splitting graph of a non-empty chain-free clause must have a root constraint.
%\item \label{lemma:subgraph}
%$H_\clause$ is always a sub-graph of $G_\clause$.
\item \label{lemma:hroot}
A non-empty $H_\clause$ must have a root.
\item\label{lemma:alwaysroot}
If a constraint of $\clause$ is a root $H_\clause$, 
then its successor may appear in $H_{\clause'}$ only as a root (or is removed if it became chain-free due to the split). 
Further, an outer side of a root of $H_\clause$
remains an outer side of its successor in $H_{\clause'}$. 
\item\label{lemma:outerdown}
The successor of an outer side either stays the same or is a suffix of the original. 
\item\label{lemma:innerorouter}
If the successor of an inner side of a root is strictly longer (has more varialbes) than the predecessor,
then an outer side of some root is shorter then its predecessor.
\end{enumerate}
\end{lemma}
\begin{proof}
\item[\ref{lemma:root}]
By contradiction, assume that there is no root constraint in a chain-free clause. 
That means that there is an edge in the splitting graph leading from each side of a constraint. 
Define high-level edges between sides of constraints such that there is an edge from $s$ to $s'$ if and only if there is an edge in the splitting graph from a position inside $s$ to a position inside $s'$.
By our initial assumption, every constraint side has an incoming edge, which implies that there is a cycle $(s_0,s_1),(s_1,s_2),\ldots,(s_{n-1},s_n),s_n = s_0$ constructed from the high-level edges. 
We will show that existence of this cycle implies existence of a chain in the splitting graph. 
By the definition of the high-level edges and of the splitting graph, 
each edge $(s_i,s_{i+1})$ implies existence of three positions $p_i,p''_i,p'_i$ such that $e_i = (p_i,p_i')$ is an edge of the splitting graph, $p_i$ is a position of $s_i$, $p_i'$ is a position of $s_{i+1}$, and $p''_i$ is opposing $p_i$ and has the same label as $p_i'$. 
Because $p_{(i+n) \modulo ({n+1})}',0\leq i \leq n$ 
is also a position of $s_i$, 
the splitting graph has also the edge 
$e_i' = (p_{(i+n) \modulo ({n+1})}',p_i)$, 
end the edges $e_1',\ldots,e_n'$ are a chain in the splitting graph.
This contradicts the assumption that the splitting graph is chain-free.
\item[\ref{lemma:hroot}]
$H_\clause$ is created from  sub-graph by removing constraints, by definition.
So it is a splitting graph of a subset of $\clause$. 
Since $\clause$ is chain-free, its subsets is also chain-free, and therefore $H_\clause$ must have a root due to Point \ref{lemma:root} above.
\item[\ref{lemma:alwaysroot}]
Due to the fact that we never add a constraint to $H_\clause'$ which did not have its predecessor in $H_\clause$. 
Being a root means that the variables on the outer side have only single occurrence in $H_\clause$ (the one inside the outer side). 
%
Such variables cannot travel anywhere else due to a splitting step (can be seen from the definition of splitting) and therefore stay roots.
\item[\ref{lemma:outerdown}]
Because root positions do not appear anywhere else in $H_{\clause}$, 
the outer side can never get affected by substitution from splitting another constraint.
Hence, by definition of splitting, it can either stay the same, or the first variable ($y$ in the case of left split) gets cut off. Notice that the constraint resulting from the left split that contains $y$ is concatenation free and therefore does not appear in $H_{\clause'}$ at all. Analogously for the right split.
\item\ref{lemma:innerorouter}
An inner side could have been made longer only due to substitution of a variable due to a split. Suppose that it was a left split (the case of the right split is analogous), hence $x$ was substituted by $x_1$ and $x_2$.
The occurrence that was replaced by $x_1\concat x_2$ in the result was not the one explicitly mentioned in the left split (because that one does not lead to creating a term $x_1\concat x_2$). Hence $x$ was occurring multiple times and so it is not appearing on the outer side of any root constraint. It must thus appear only on the inner side of the constraint on which  the split is applied. Notice that by the definition of split, the side of the constraint opposite the position of $x$ explicit in the rule gets shorter under the assumption that $x$ does not appear in it. Since it is the outer side, $x$ indeed cannot appear in it. It is therefore the sought outer side of a root constraint that got shorter. 
%
\qed
\end{proof}
With Lemma~\ref{lemma:aux1} in hand, we are ready to show termination of Phase~1.
\begin{lemma}
Phase~1 terminates.
\end{lemma}
\begin{proof}
Let us annotate each clause $\clause$ with a measure $m(\clause) = (l,o,i)$ where 
\begin{itemize}
\item
$l$ equals the number of the original constraints minus the number of times a new constraint becomes a root constraint. 
\item
$o$ equals the sum of the lengths of the outer sides of roots in $H_\clause$, and
\item
$i$ equals the sum of the lengths of the inner sides of roots in $H_\clause$.
\end{itemize}
%
Let $(l,o,i)<(l',o',i')$ if and only if
$$
(l < l') \lor (l = l' \land o < o') \lor (l = l' \land o = o' \land i < i') 
$$ 
Notice that $0\leq l \leq n_0$, where $n_0$ is the number of the original constraints in $\clause$, is an invariant of the algorithm 
(i.e., at most as many times a root constraint is created as there are constraints in the original clause). 
Notice that 1) introducing one new root constraint means decreasing the number of constraint in the reminder graph, and
2) splitting never increases the number of constraints in the reminder graph. 
Therefore $m(\clause)$ is bounded from below by $(0,0,0)$ for all clauses created in Phase~1.
We will show termination of Phase~1 by showing that for a clause $\clause'$ created from $\clause$ by splitting, $m(\clause') < m(\clause)$:

If a constraint from the reminder graph became a root constraint, 
then $l > l'$ and we are done.
The case $l < l'$ can never happen by definition of $l$.
%
If $l = l'$ and some outer side got shorter, then we have $o > o'$ and we are done. 
Since $l = l'$, the set of roots is the same as before and hence it is not possible that $o < o'$. This is because the variables in outer sides have only a single occurrence in the reminder graph (because outer sides consist of positions that are leaves of the reminder graph), and hence it is not possible to achieve that some constraint side gets longer by substituting such variable by splitting of constraint in the reminder graph (be definition of split).
%
If $l = l'$ and $o = o'$, then the set of leaves is the same, but this means that $i$ must have decreased by Lemma~\ref{lemma:aux1}, hence we have that $i > i'$. This concludes the proof of termination of Phase~1.
\qed
\end{proof}

Our argument that Phase~2 terminates is based on that Phase~1 returns clauses that satisfy certain special properties. 
We note that these properties imply that the clauses fall into the straight line fragment of \cite{BL16}.
%
However, we do not use the algorithm from \cite{BL16}. 
Our algorithm allows to apply splitting in any order, which is much more liberal than in \cite{BL16}.
%
The main difference is that \cite{BL16} must \emph{explicitly use} certain ordering of constraints to guide the computation (roughly corresponding to restricting the choice of splitting steps), while we only use an \emph{existence} of that ordering to prove termination, but do not restrict the choice of splitting steps in the algorithm. 

We will define a partial ordering of the constraints of the clause $\clause$ output by Phase~1. Consider the sequence of clauses $\clause_0,\ldots,\clause_n = \clause$  
such that $\clause_0$ is an initial clause and $\clause_i$ is created from $\clause_0$ in Phase~1 by a splitting step. Consider also the sequence of remainder graphs $H_{\clause_0},\ldots,H_{\clause_n}$ associated with these clauses during Phase~1. 
%
Let $\drop_i,1\leq i \leq n$ be the set of successors of the constraint $\constr$ of $\clause_{i-1}$  that was split in the $i$th step that are concatenation-free and hence are removed from the reminder graph $H_{\clause_{i}}$ ($\drop_i$ contains one or two elements, by the definition of split). 
%
Let the side of a constraint in $\drop_i$ that is a successor of the outer side of the predecessor $\constr$ ($\constr$ was a root, hence it has an outer side, otherwise the splitting would not be applied on it) be also called outer side.
%
Let $\clause(i)$ be the set of constraints in $\clause$ that are successors of constraints in  $\drop_i$ (we extend the relation of being successor by closing under transitivity). 
%
Further, let the side of a constraint in $\clause(i)$ that is  a successor of the outer side of the predecessor constraint in $\drop_i$ be called outer side.
%
We will use several auxiliary observations about these notions to prove termination of Phase~2.
\begin{lemma}[Initial conditions]
\label{lemma:init}
\begin{enumerate}
\item\label{lemma:cover}
$\{\clause(i)\mid 0\leq i \leq n\}$ covers the constraints of $\clause$,
\item\label{lemma:singleton}
the outer side of every constraint of $\clause$ is a singleton,
\item\label{lemma:notupwards}
the outer side of every constraint in $\clause(i)$ does not appear in any constraint from $\clause(j),j>i$ 
and in any other constraint in $\clause(i)$,
\item\label{lemma:distinct}
all outer side variables of $\clause$ are pairwise different.
\end{enumerate}
\end{lemma}
\begin{proof}
\item[\ref{lemma:cover}]
Phase 1 starts with the reminder graph containing all constraints of the original formula.
All constraints of $\clause$ are successors of the constraints of the original formula (they are created by splitting from the original formula).
When a successor of a constraint of the original formula is removed from reminder graphs during Phase 1, it is added to some $\drop(i)$ and its successor will appear in $\clause(i)$. 
Phase 1 ends with the reminder graph empty, so every constraint in $\clause$ has a predecessor that was removed from reminder graphs and hence it belongs to some $\clause(i)$.
\item[\ref{lemma:singleton}]
When a constraint is added to $\drop_i$, it is concatenation-free, so its outer side is a singleton.
%
Since it is an outer side, its variable $z$ does not appear in the reminder graph.
%
All the further substitution happens with constraints and variables of the reminder graphs only, so the substitutions made by splitting steps cannot affect $z$. The outer side thus stays $z$ until the end of Phase 1.
\item[\ref{lemma:notupwards}]
We just argued that outer sides of constraints do not change from their addition to $\drop_i$ until the end of Phase 1. At that point, the variable $z$ at the outer side does not appear in the reminder graph, since it is an outer side of the leaf. It will never propagated to other constraints during Phase 1 because further splitting takes place only inside reminder graphs.  
Constraints in $\clause(j),j> i$ are successors of constraints that are after the $i$th split still in the reminder graph. Hence these predecessors of the of the constraints in $\clause(j)$ cannot contain $z$, and hence the constraints themselves cannot contain $z$ too (since $z$ does not appear in any further splitting in Phase 1). 
\item[\ref{lemma:distinct}]
This follows directly from the previous points \ref{lemma:cover}, \ref{lemma:singleton}, and \ref{lemma:notupwards}.
\qed
\end{proof}

Let $\clause = \clause'_0,\clause'_1,\ldots$ be a sequence of clauses created each from the previous by a splitting step during Phase 2.
%
We will maintain the division of constraints in $\clause$ into $\{\clause(i)\mid 0\leq i \leq n\}$ during Phase 2 by defining
$\clause(i) \defeq \clause_0'(i)$ and 
defining $\clause_{j+1}'(i)$ to consist of the successors of the constraints in $\clause_{j}'(i)$, for all $0\leq i \leq n$.
%
The observations made in Lemma~\ref{lemma:init} above are actually invariants during entire Phase 2, as expressed by the following lemma. 
\begin{lemma}[Invariant] For all $j\geq 0$ it holds that
\label{lemma:inv}
\begin{enumerate}
\item\label{lemma:cover2}
$\{\clause_j'(i)\mid 0\leq i \leq n\}$  covers the constraints of $\clause_j'$,
\item\label{lemma:singleton2}
the outer side of every constraint of $\clause_j'$ is a singleton,
\item\label{lemma:notupwards2}
the outer side of every constraint in $\clause_j'(i)$ does not appear in any constraint from $\clause(j),j>i$ 
and in any other constraint in $\clause_j'(i)$, and
\item\label{lemma:distinct2}
all outer side variables of $\clause_j$ are pairwise different.
\end{enumerate}
\end{lemma}
\begin{proof}
All the four points hold initially for $j = 0$ due to Lemma~\ref{lemma:init}. 
Assume now that they hold before split. After the split
\item[\ref{lemma:cover2}]
By the definition of $\clause_j(i)'$.
\item[\ref{lemma:singleton2}]
The condition is preserved through splitting since in a splitting step on a constraint $\constr$ with the outer side being a singleton $z$, the variable $z$ must be the one being substituted by two fresh variables $z_1,z_2$, by definition of splitting. But since point \ref{lemma:distinct2} was true, this substitution cannot affect any other outer side. 
The splitting on $\varphi$ produces two constraints, one with the outer side term $z_1$ and the other with the outer side term $z_2$.  
\item[\ref{lemma:notupwards2}]
Continuing the argumentation from the previous point,
since \ref{lemma:distinct2} was true and a constraint with an outer side in $\clause_{j-1}'(i)$ can be only replaced by two constraints with fresh variables on the outer sides in $\clause_{j}'(i)$, point \ref{lemma:notupwards2} holds.
\item[\ref{lemma:distinct2}]
Directly implied by the previous points \ref{lemma:cover2}, \ref{lemma:singleton2}, and \ref{lemma:notupwards2}.
\qed
\end{proof}
%
With the lemma above at hand, we can finish the proof.
\begin{lemma}
Phase 2 terminates.
\end{lemma}
\begin{proof}
The decreasing well founded measure we use is defined as follows.
For $j\geq 0$,  $m(\clause_j')$ is the vector $(\iota_0,\ldots,\iota_n)$ where $\iota_k$ is the sum of the lengths of the inner sides of constraints in $\clause_j'(k)$.  
%
The ordering $<$ on vectors is the usual lexicographic ordering (the $n$th position is the most significant).
%
Obviously, $m(\clause_j')\geq 0^n$ for all $j$.
%
We will argue that $m(\clause_j')>m(\clause_{j+1}')$ for all $j\geq 0$:

Assume that the splitting step has split a constraint in $\clause_j'(k)$.
%
By the invariant expressed by Lemma~\ref{lemma:inv}, 
the substitution in the split can affect (and increase their length) only inner sides of constraints at the level strictly higher than $j$.
At the level $j$, by the definition of split, a constraint with the inner side of the length $n$ is replaced by two constraints with the inner sides of the length $1$ and $n-1$, 
therefore the sum of the inner sides at the level $j$ decreases at least by $1$.
This means that $m(\clause_j')>m(\clause_{j+1}')$ and we are done.
\qed
\end{proof}

Let us summarise the proof.
Since Phase 1 and Phase 2 terminate, the algorithm terminates. Since it only uses splitting to modify the formula and since by definition, splitting produces an equisatisfiable formula, the result is equisatisfiable.
Since splitting preserves chain-freeness, the resulting formula is chain-free. 
Since the only termination condition of Phase 2 is concatenation-freeness and Phase 2 terminates, the resulting formula is concatenation-free. This concludes the proof of Theorem~\ref{theorem:splitting}. 


==> sections/undecidability_proof_journal.tex <==
%\section{Proof of Lemma~\ref{lemma:undecidability}}
%\label{proof:undecidability}
\begin{proof}[Lemma~\ref{lemma:undecidability}]
\newcommand{\id}{\mathit{Id}}
We will show the lemma by reduction of undecidability of constraints of the form $\transducer(x,x)$  %\cite{morvan,Chen:2019}\lukas{is the reference right?}.
%
Let $\Phi$  be a chaining conjunction of relational constraints.
%
We will show how any constraint $\transducer(x,x)$ can be translated into an equivalent constraint $\Phi'$ with the same skeleton as $\Phi$.
%

Let $\Psi = \rel_1(\term_1,\term_1') \land \cdots \land \rel_n(\term_n,\term_n')$ be a conjunction of a smallest sub-set of the relational constraints of $\Phi$ which is chaining.
%
Let $x_i, 1\leq i \leq n$, be the variable which labels the position within $t_i$ that is a part of the chain. 
%
$\Phi'$ will be constructed to be equivalent to 
$\transducer(x_1,x_{2}) \land x_{2} = x_3 \land \cdots \land x_n = x_1$.


Let $\sharp$ be a symbol outside the alphabet $\Sigma$, let $\Sigma_\sharp$ denote $\Sigma\cup\{\sharp\}$. 
%
%Let $k_i$ be the number of occurrences of $x_i$ in $t_i$ and let $l_i$ be the number of occurrences of $x_i$ in $t_{i-1}'$ or in $t_n'$ if $i = 1$.
%
Then the new constraint $\Phi'$ is created from $\Psi$ by:

\begin{enumerate}
%\item 
%introducing the membership constraint $x_i\in \automaton_{\Sigma^*.\{\sharp\}}$ with $\langof{\automaton_{\Sigma^*.\{\sharp\}}} = \Sigma^*.\{\sharp\}$ for all $1\leq i \leq n$,
%\item 
%introducing a membership constraint $y\in \automaton_\epsilon$ with $\langof{\automaton_\epsilon} = \{\epsilon\}$ for all variables $y$ other then $x_1,\ldots,x_n$.
\item 
Introducing membership constraints $x_i\in \automaton, 1\leq i \leq n$ with $\langof{\automaton} = \Sigma^*\concat\{\sharp\}$ (this is to make the borders of the variables $x_i$ visible).
\item 
Introducing membership constraints $y\in \automaton_\epsilon$ with $\langof{\automaton_\epsilon} = \{\epsilon\}$ for all variables $y$ other then $x_1,\ldots,x_n$ (this is to ``erase'' these variables from the valuations of $t_1,\ldots,t_n$).
\item 
Replacing every $\rel_i$ in $\Psi$ by $\rel_i'$ where  
\begin{enumerate}
\item 
$\relof{\rel_1'} = \relof{\transducer} \concat \{(\sharp,\sharp)\} \concat \Sigma_\sharp^*\times \Sigma^*_\sharp$ and
\item
$\relof{\rel_i'} = \id \concat \{(\sharp,\sharp)\} \concat \Sigma_\sharp^*\times \Sigma_\sharp^*$ for $1 < i \leq n$, $\id$ being the identity on $\Sigma^*$. 
\end{enumerate}
Here (a) together with (1) and (2) assures that the first track of $\transducer$ is mapped at the first occurence of $x_1$ in $t_1$ and the second track at the first occurence of $x_2$ in $t_2$ (it cannot be multiple occurrences of $x_1$ or of $x_2$ due to the use $\sharp$ as a variable delimiter in (1) and (3a)); and (3b) together with (1) and (2) encodes the equalities $x_i = x_{i+1}$, since they ensure that the left track of the identity transducer in $\rel_i'$ is mapped at $x_i$ and the right track at $x_{i+1}$. 
\item 
Replacing all the relational constraints $\rel(t,t')$ of $\Phi$ outside $\Psi$ by $\rel'(t,t')$ where $\relof{\rel'} =\Sigma^*\times\Sigma^*$ (to make them irrelevant).
\end{enumerate}
%
%The constraint $\Phi'$ was designed for this to hold, particularly,
%the role of the $\automaton_\epsilon$-membership constraints was to eliminate assignments to variables other then $x_1,\ldots,x_n$,
%the part of the primed relational constraints $\{(\sharp,\sharp)\} \concat \Sigma_\sharp^*\times \Sigma^*_\sharp$ was added to eliminate the effect of possible multiple occurrences of the variables $x_i$ in terms,
%and the $\Sigma^*\times\Sigma^*$ constraints outside $\Psi$ were chosen to eliminate any influence of the part of $\Phi$ outside the chain.

Last, to show that 
$\Phi' \equiv \transducer(x_1,x_{2}) \land x_{2} = x_3 \land \cdots \land x_n = x_1$ indeed holds,
it must be argued that every $x_i,2\leq i \leq n$ appears in $\Psi$ only in $t_i$ and $t'_{i-1}$ and
$x_1$ appears in $\Psi$ only in $t_1$ and $t'_{n}$ (otherwise the cycle of variable occurences related by $\transducer$ and $\id$ by relations from point (3) above could be cut short, resulting in a shorter cycle of occurences related by $\id$ only).
This may be shown from the minimality of $\Psi$, by contradiction: if $x_i$ appeared somewhere else, we could shorten the chain, and $\Psi$ would not be minimal. Particularly, take w.l.o.g. $x_1$ as the variable contradicting the claim. There are two options:
\begin{itemize}
\item
$x_1$ appears also in some $t_m, 1< m \geq n$. Then, in the case $m < n$, the splitting graph has an edge from $x_1$ in $t_m$ to the $x_{m+1}$ in $t_{m+1}$ and $x_n$ in $t_n$ has an edge to the $x_1$ in $t_m$, closing a shorter chain that bypasses the first $m-1$ edges of the original. Otherwise, if $m=n$, then due to the occurence of $x_1$ in $t_{n'}$, there is a self-loop on the occurence of $x_1$ in $t_n$ (as well as on the occurence in $t_{n'}$).
Both cases contradict the assumed minimality of $\Psi$.
\item
$x_1$ appears also in some $t_m',1 \leq m > n$. But then the splitting graph has an edge from the occurrence of $x_m$ in $t_m$ to the occurrence of $x_1$ in $t_1$, closing a shorter chain that bypasses the last $n-m +1$ edges of the original, which again contradicts the minimality of $\Psi$.
\end{itemize}
\qed
\end{proof}




